The extreme HBL behaviour of Markarian 501 during 2012

A multiwavelength campaign was organized to take place between March and July of 2012. Excellent temporal coverage was obtained with more than 25 instruments, including the MAGIC, FACT and VERITAS Cherenkov telescopes, the instruments on board the Swift and Fermi spacecraft, and the telescopes operated by the GASP-WEBT collaboration. Mrk 501 showed a very high energy (VHE) gamma-ray flux above 0.2 TeV of $\sim$0.5 times the Crab Nebula flux (CU) for most of the campaign. The highest activity occurred on 2012 June 9, when the VHE flux was $\sim$3 CU, and the peak of the high-energy spectral component was found to be at $\sim$2 TeV. This study reports very hard X-ray spectra, and the hardest VHE spectra measured to date for Mrk 501. The fractional variability was found to increase with energy, with the highest variability occurring at VHE, and a significant correlation between the X-ray and VHE bands. The unprecedentedly hard X-ray and VHE spectra measured imply that their low- and high-energy components peaked above 5 keV and 0.5 TeV, respectively, during a large fraction of the observing campaign, and hence that Mrk 501 behaved like an extreme high-frequency- peaked blazar (EHBL) throughout the 2012 observing season. This suggests that being an EHBL may not be a permanent characteristic of a blazar, but rather a state which may change over time. The one-zone synchrotron self-Compton (SSC) scenario can successfully describe the segments of the SED where most energy is emitted, with a significant correlation between the electron energy density and the VHE gamma-ray activity, suggesting that most of the variability may be explained by the injection of high-energy electrons. The one-zone SSC scenario used reproduces the behaviour seen between the measured X-ray and VHE gamma-ray fluxes, and predicts that the correlation becomes stronger with increasing energy of the X-rays.

==> notes/authors_last_AA.tex <==
% authors 16.09.2014  Format AA
%
\author{
J.~Aleksi\'c\inst{1} \and
S.~Ansoldi\inst{2} \and
L.~A.~Antonelli\inst{3} \and
P.~Antoranz\inst{4} \and
A.~Babic\inst{5} \and
P.~Bangale\inst{6} \and
U.~Barres de Almeida\inst{6,}\inst{25} \and
J.~A.~Barrio\inst{7} \and
J.~Becerra Gonz\'alez\inst{8,}\inst{26} \and
W.~Bednarek\inst{9} \and
E.~Bernardini\inst{10} \and
B.~Biasuzzi\inst{2} \and
A.~Biland\inst{11} \and
O.~Blanch\inst{1} \and
S.~Bonnefoy\inst{7} \and
G.~Bonnoli\inst{3} \and
F.~Borracci\inst{6} \and
T.~Bretz\inst{12,}\inst{27} \and
E.~Carmona\inst{13} \and
A.~Carosi\inst{3} \and
P.~Colin\inst{6} \and
E.~Colombo\inst{8} \and
J.~L.~Contreras\inst{7} \and
J.~Cortina\inst{1} \and
S.~Covino\inst{3} \and
P.~Da Vela\inst{4} \and
F.~Dazzi\inst{6} \and
A.~De Angelis\inst{2} \and
G.~De Caneva\inst{10} \and
B.~De Lotto\inst{2} \and
E.~de O\~na Wilhelmi\inst{14} \and
C.~Delgado Mendez\inst{13} \and
F.~Di Pierro\inst{3} \and
D.~Dominis Prester\inst{5} \and
D.~Dorner\inst{12} \and
M.~Doro\inst{15} \and
S.~Einecke\inst{16} \and
D.~Eisenacher\inst{12} \and
D.~Elsaesser\inst{12} \and
A.~Fern\'andez-Barral\inst{1} \and
D.~Fidalgo\inst{7} \and
M.~V.~Fonseca\inst{7} \and
L.~Font\inst{17} \and
K.~Frantzen\inst{16} \and
C.~Fruck\inst{6} \and
D.~Galindo\inst{18} \and
R.~J.~Garc\'ia L\'opez\inst{8} \and
M.~Garczarczyk\inst{10} \and
D.~Garrido Terrats\inst{17} \and
M.~Gaug\inst{17} \and
N.~Godinovi\'c\inst{5} \and
A.~Gonz\'alez Mu\~noz\inst{1} \and
S.~R.~Gozzini\inst{10} \and
D.~Hadasch\inst{14,}\inst{28} \and
Y.~Hanabata\inst{19} \and
M.~Hayashida\inst{19} \and
J.~Herrera\inst{8} \and
J.~Hose\inst{6} \and
D.~Hrupec\inst{5} \and
W.~Idec\inst{9} \and
V.~Kadenius \and
H.~Kellermann\inst{6} \and
M.~L.~Knoetig\inst{11} \and
K.~Kodani\inst{19} \and
Y.~Konno\inst{19} \and
J.~Krause\inst{6} \and
H.~Kubo\inst{19} \and
J.~Kushida\inst{19} \and
A.~La Barbera\inst{3} \and
D.~Lelas\inst{5} \and
N.~Lewandowska\inst{12} \and
E.~Lindfors\inst{20,}\inst{29} \and
S.~Lombardi\inst{3} \and
F.~Longo\inst{2} \and
M.~L\'opez\inst{7} \and
R.~L\'opez-Coto\inst{1} \and
A.~L\'opez-Oramas\inst{1} \and
E.~Lorenz\inst{6} \and
I.~Lozano\inst{7} \and
M.~Makariev\inst{21} \and
K.~Mallot\inst{10} \and
G.~Maneva\inst{21} \and
K.~Mannheim\inst{12} \and
L.~Maraschi\inst{3} \and
B.~Marcote\inst{18} \and
M.~Mariotti\inst{15} \and
M.~Mart\'inez\inst{1} \and
D.~Mazin\inst{6} \and
U.~Menzel\inst{6} \and
J.~M.~Miranda\inst{4} \and
R.~Mirzoyan\inst{6} \and
A.~Moralejo\inst{1} \and
P.~Munar-Adrover\inst{18} \and
D.~Nakajima\inst{19} \and
V.~Neustroev\inst{20} \and
A.~Niedzwiecki\inst{9} \and
M.~Nievas Rosillo\inst{7} \and
K.~Nilsson\inst{20,}\inst{29} \and
K.~Nishijima\inst{19} \and
K.~Noda\inst{6} \and
R.~Orito\inst{19} \and
A.~Overkemping\inst{16} \and
S.~Paiano\inst{15} \and
M.~Palatiello\inst{2} \and
D.~Paneque\inst{6} \and
R.~Paoletti\inst{4} \and
J.~M.~Paredes\inst{18} \and
X.~Paredes-Fortuny\inst{18} \and
M.~Persic\inst{2,}\inst{30} \and
J.~Poutanen\inst{20} \and
P.~G.~Prada Moroni\inst{22} \and
E.~Prandini\inst{11,}\inst{31} \and
I.~Puljak\inst{5} \and
R.~Reinthal\inst{20} \and
W.~Rhode\inst{16} \and
M.~Rib\'o\inst{18} \and
J.~Rico\inst{1} \and
J.~Rodriguez Garcia\inst{6} \and
T.~Saito\inst{19} \and
K.~Saito\inst{19} \and
K.~Satalecka\inst{7} \and
V.~Scalzotto\inst{15} \and
V.~Scapin\inst{7} \and
C.~Schultz\inst{15} \and
T.~Schweizer\inst{6} \and
S.~N.~Shore\inst{22} \and
A.~Sillanp\"a\"a\inst{20} \and
J.~Sitarek\inst{1} \and
I.~Snidaric\inst{5} \and
D.~Sobczynska\inst{9} \and
A.~Stamerra\inst{3} \and
T.~Steinbring\inst{12} \and
M.~Strzys\inst{6} \and
L.~Takalo\inst{20} \and
H.~Takami\inst{19} \and
F.~Tavecchio\inst{3} \and
P.~Temnikov\inst{21} \and
T.~Terzi\'c\inst{5} \and
D.~Tescaro\inst{8} \and
M.~Teshima\inst{6} \and
J.~Thaele\inst{16} \and
D.~F.~Torres\inst{23} \and
T.~Toyama\inst{6} \and
A.~Treves\inst{24} \and
P.~Vogler\inst{11} \and
M.~Will\inst{8} \and
R.~Zanin\inst{18} \and
}
\institute { IFAE, Campus UAB, E-08193 Bellaterra, Spain
\and Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy
\and INAF National Institute for Astrophysics, I-00136 Rome, Italy
\and Universit\`a  di Siena, and INFN Pisa, I-53100 Siena, Italy
\and Croatian MAGIC Consortium, Rudjer Boskovic Institute, University of Rijeka and University of Split, HR-10000 Zagreb, Croatia
\and Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany
\and Universidad Complutense, E-28040 Madrid, Spain
\and Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, Tenerife, Spain
\and University of \L\'od\'z, PL-90236 Lodz, Poland
\and Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany
\and ETH Zurich, CH-8093 Zurich, Switzerland
\and Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany
\and Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, E-28040 Madrid, Spain
\and Institute of Space Sciences, E-08193 Barcelona, Spain
\and Universit\`a di Padova and INFN, I-35131 Padova, Italy
\and Technische Universit\"at Dortmund, D-44221 Dortmund, Germany
\and Unitat de F\'isica de les Radiacions, Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain
\and Universitat de Barcelona, ICC, IEEC-UB, E-08028 Barcelona, Spain
\and Japanese MAGIC Consortium, KEK, Department of Physics and Hakubi Center, Kyoto University, Tokai University, The University of Tokushima, ICRR, The University of Tokyo, Japan
\and Finnish MAGIC Consortium, Tuorla Observatory, University of Turku and Department of Physics, University of Oulu, Finland
\and Inst. for Nucl. Research and Nucl. Energy, BG-1784 Sofia, Bulgaria
\and Universit\`a di Pisa, and INFN Pisa, I-56126 Pisa, Italy
\and ICREA and Institute of Space Sciences, E-08193 Barcelona, Spain
\and Universit\`a dell'Insubria and INFN Milano Bicocca, Como, I-22100 Como, Italy
\and now at Centro Brasileiro de Pesquisas F\'isicas (CBPF\textbackslash MCTI), R. Dr. Xavier Sigaud, 150 - Urca, Rio de Janeiro - RJ, 22290-180, Brazil
\and now at NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA and Department of Physics and Department of Astronomy, University of Maryland, College Park, MD 20742, USA
\and now at Ecole polytechnique f\'ed\'erale de Lausanne (EPFL), Lausanne, Switzerland
\and now at Institut f\"ur Astro- und Teilchenphysik, Leopold-Franzens- Universit\"at Innsbruck, A-6020 Innsbruck, Austria
\and now at Finnish Centre for Astronomy with ESO (FINCA), Turku, Finland
\and also at INAF-Trieste
\and also at ISDC - Science Data Center for Astrophysics, 1290, Versoix (Geneva)
}


==> notes/polarization.tex <==

\subsection{Polarization}


   \begin{figure}
   \centering
   \includegraphics[width=23pc]{figures3/Mrk501_polarization_all.eps}
   \caption{Electric vector polarization angle and polarization
     degree during the multi-instrument campaign of Mrk~501 in
     2012. The correspondence between the instruments and the measured
     quantities is given in the legend. Further details about
     these measurements are given in Section
     \ref{optical:description}. The blue vertical line is represents 
     the day of the VHE flare (MJD=56087).
   }
      \label{fig:polar}
   \end{figure}



